ViLPAct: A Benchmark for Compositional Generalization on Multimodal Human Activities

We introduce ViLPAct, a novel vision-language benchmark for human activity planning. It is designed for a task where embodied AI agents can reason and forecast future actions of humans based on video clips about their initial activities and intents in text. The dataset consists of 2.9k videos from \charades extended with intents via crowdsourcing, a multi-choice question test set, and four strong baselines. One of the baselines implements a neurosymbolic approach based on a multi-modal knowledge base (MKB), while the other ones are deep generative models adapted from recent state-of-the-art (SOTA) methods. According to our extensive experiments, the key challenges are compositional generalization and effective use of information from both modalities.

==> backup.tex <==
\begin{table}[!htb]
\centering


\scalebox{0.7}{\begin{tabular}{l|cc}
\hline
\multirow{2}{*}{Feature} & \multicolumn{}{c}{\multirow{2}{*}{num}} & \multirow{2}{*}{size} \\
 & \multicolumn{}{c}{} &  \\ \hline
action visual prototype feat   &    157                  &[1024,]\\
action textual prototype feat   &   157                  &[768,]\\
intent feat  &  2402*2  & [768,]  \\
video-level visual feat& 2402 + 12118&[1024,]\\
frame-level visual feat& 2402 + 12118&  [frames//8, 1024]\\
\hline
\end{tabular}}
\caption{Features in MKB / training set}
\label{table:Features in KB}
\vspace{-5mm}
\end{table}

==> dataset_copy.tex <==
%We select videos from Charades \cite{sigurdsson2016hollywood} and collect intents and action  sequences on Amazon Mechanical Turk. For each video of interest, we collect intentions of action sequences from the video via crowdsourcing. With the refinement, we include 2912 videos in the dataset, which is split into a training/validation/test sets with ratios of 70\%, 10\%, 20\%. On the training dataset, we build an MKB by incorporating structural and conceptual information. On the test dataset, we collect a set of multi-choice questions and answers for the evaluation task. 
We add intents to the videos with long action sequences in \charades \cite{sigurdsson2016hollywood} via crowdsourcing. As there are multiple plausible future action sequences to meet an intent based on a given initial video clip, we construct a test set with multi-choice questions to let models select the most reasonable one among all options. In order to encourage models to focus on tackling the problem of compositional generalization, we do not provide multi-choice questions for training but only videos and action sequences annotated with intents, because we do not want models to merely learn the differences between true answers and incorrect answers generated by a particular method. % To compare different types of baselines, we build an MKB on the training set by incorporating structural and conceptual information. 

\subsection{Video Selection}
\charades is a large-scale video dataset of daily indoors activities collected via Amazon Mechanical Turk. The average length of videos is approximately 30 seconds. It involves interactions with 46 object classes and contains 157 action classes, which are also referred to as actions for short. Each action is represented as a verb phrase, such as "pouring into cup".  This dataset is chosen because i) it contains sufficient number of long action sequences of human daily activities; ii) the intents are easily identifiable as the activities in the videos are based on scripts; iii) there are rich annotations of videos that can be leveraged for dataset construction.  

Each video of \charades is annotated with actions from at least one action sequence. The starting and ending points of an action are labeled, but it is not clear which actions jointly meet an intent. Therefore, we have implemented an algorithm to automatically extract action sequences with clear intents from videos. For each video, the algorithm aims to identify a sequence of semantically coherent actions, which interacts with the same or relevant objects. More details of the implementation can be found in Appendix \ref{alg:cap}.

Following~\cite{ng2020forecasting}, we consider the first 20\% of a video as its initial visual state and aim to forecast future actions appearing in the remaining part of the video for a given intent. To have at least one future actions per video, we keep only the videos, which contain at least one action sequence comprising more than three actions. As a result, we obtain 2912 such videos. Each video is associated with one action sequence with length longer than three. The whole dataset is further split into training/validation/test sets with ratios of 70\%, 10\%, 20\% for experiments.

In order to assess the quality of extracted action sequences in the selected videos, we randomly sampled 100 videos from the test set for manually inspection. %The primary action sequence of each video is evaluated in terms of three criteria: i) if all actions of a sequence occur in the video; ii) if the actions of a sequence appear in the same order as that in the video; iii) if a sequence has any actions missing between the first and the last action. In total, 
We found out that 94 videos have all actions of their action sequences covered in the video. The actions of 92 videos appear in the same order as that in the videos. And 85 videos have no actions missing between the first and the last action of their sequences. Thus, the quality of those action sequences is adequate for VL planning evaluation.

%The manual evaluation results are shown in the Table \ref{table:action seq quality}.
%\begin{table}[htb]
 %   \centering
 %   \scalebox{0.5}{\begin{tabular}{|c|c|c|c|}
 %   \hline
  %   all actions in vid (\%) & all actions in order (\%) & no missing actions (\%) & qualified action sequences\\ \hline
  %  94 & 92 & 85 & 82\\ \hline
 %   \end{tabular}}
 %   \caption{Action sequence Quality}
 %   \label{table:action seq quality}
%\end{table}

%Since Charades is large-scale and comprehensive, the video usually contains more than one activity. Here, we define an activity annotation in the video as a sequence of actions. In order to simplify our task setting, we only consider one single activity with a clear intent in the video. To achieve the goal, we design the activity (action sequence) extraction algorithm to organize the temporal activity chains from the action set of the charades video. This algorithm uses a greedy search that explores an action sequence by expanding the most promising action in a limited set. It uses text similarity, temporal relevance, and topic matching between two actions to find the most possible next action in the candidate set. The details of the implementation is shown in Appendix \ref{alg:cap}.

%By applying the algorithm, we filter out 223 videos that don't have action set labels and 6622 videos that don't contain action sequences longer than 4. After filtering we get about 3003 videos, each of which consists of some action sequences that contain more than 4 actions. For each video, we randomly selected one action sequence as the main activity. These examples contain 2371 non-repetitive action sequences, covering 148 of all 157 action classes from the original Charades. 

%We randomly split the 3003 videos into 2402 train data and 601 test data. The train data was used to construct the KB, and the test data was used to construct our evaluation task. For the evaluation tasks, we filtered out videos that were of poor quality or didn't contain future actions that started after 20\% of the time of the video. Final 510 videos were left for the evaluation task. 


\subsection{Intent Annotation}
According to Cambridge Dictionary, \textit{intent} is "something that you want and plan to do"\footnote{https://dictionary.cambridge.org/}. Philosophers distinguish between future-directed intents and present-directed ones~\cite{cohen1990intention}. The former guides planning of actions, while the latter causally produces behavior. As the focus of this work is planning of actions, we encourage crowd-workers to provide future-directed intents.

We recruit university students to annotate videos with future-directed and present-directed intents. Each student is provided with a full video clip and the associated action sequence. They are instructed to answer the question \textit{what the person wants to do by taking the actions in the video}. Every student needs to write down two intents. One of them describes which activity the person intents to take, such as "drink a glass of water". The other one needs to be at a higher-level, such as "quench the thirst". Thus, the students are encouraged to provide future-directed intents by differentiating them from the ones causally leading to behaviours. In addition, students are instructed to write both intents in the form of \textit{verb + something} to facilitate normalization of collected intents.
%We randomly assign 3 crowd workers to write the intent of given action sequence aligned with the video. The intent was specified as the format of a phrase consisting of a verb and an entity, such as "eat a sandwich" and "clean the kitchen". The workers are instructed by the prompt of The person has  taken the above actions in the video because he/she wants to do what?" after watching the video and checking the action sequence. To finalize the annotated intent of each video, each three intents from the same video are firstly normalized to the desired format in the crowdsourcing instruction. Then, the most reasonable intent from each three intents is chosen by the expert

\subsection{Multi-Choice Questions for Planning}
\label{sec:multichoice}
Given the first 20\% of a video as the initial state $\vs$ and a future-directed intent $\vg$ in text, the planning evaluation task is to choose the most plausible future action sequence $\va^f$ from six available choices. We determine the initial action sequence $\va^i$ by checking if an action of a sequence starts before the end time of the initial state. To build such a dataset, we extended the test set with adversarially generated incorrect answers. As the automatic approach may generate reasonable action sequences, we recruited Amazon Mechanical Turk\footnote{https://www.mturk.com/} (AMT) turkers to manually check all answers and determine the most plausible ones as the correct answers. Figure \ref{fig:examples}
in Appendix \ref{appendix:task_example} shows an example of our planning task.

\paragraph{Generation of Incorrect Answers.} We adapt \textit{Adversarial Matching} (AM) \cite{zellers2019recognition} to turn the action sequence generation task into a multi-choice test. The key idea of using AM in this work is to substitute an action of an observed action sequence for an alternative action, which is relevant to the preceding actions and is not overly similar to the action to replace. As many videos in the test set have only one future action, the AM algorithm is extended to optionally insert a future action to generate an answer candidate.

More specifically, given the initial state, the action sequence, and the intent $(\vs, \va, \vg)$ of a video, where $\va = (\va^i, \va^f)$, the algorithm performs either an insertion or substitution to generate an answer candidate. It starts with randomly deciding if it applies substitution or insertion. If insertion is chosen, it inserts an action randomly selected from the 157 actions at a position, which is randomly picked after the last action in $\va^i$. If substitution is chosen, we feed the initial action sequence $\va^i$ to \bert \cite{devlin2018bert} and use the representation of the special classification token, CLS, as the representation of $\va^i$. Then we apply \bert to turn each action into a vector by using the corresponding CLS representation. We randomly pick a future action $a_i$ in $\va^f$ and compute the score of a candidate action $a_j$ by using the following equation.
%We first apply \textbf{Adversarial Matching} \cite{zellers2019recognition}, a QA-pair assignment algorithm to match both positive and negative answers.Statically, we concluded that the quality of crowd-sourced result achieve the best when $\lambda = 0.7$ in 
\begin{equation}
s(a_j)=\log(P_{sim}(\va^i,a_j))+\lambda \log(1-P_{sim}(a_i,a_j))
\end{equation}
where $P_{sim}()$ is defined as cosine similarity. We set $\lambda = 0.7$ to find an optimal tradeoff between the obfuscation level of an incorrect answer and the probability of being a reasonable answer. We repeat the algorithm until we generate five answer candidates.
%where $w$ is a weight matrix of maximum-weight bipartite matching, $P$ is $P(BERT)$  for $P_{rel}$ and $P_{sim}$ for reference action $r$ and candidate action $c$. However, \textbf{Adversarial Matching} could be limited when the action sequence doesn't contain many actions. Hence, for those short action sequence candidates, we randomly insert one of the actions in the original 157 Charades action classes to the action sequences. By combining these two methods, we increase the diversity of generated negative answers. 

%\paragraph{\textbf{Overview}} When we get a high-level intent of each video, we could continue designing our planning crowdsourcing task, which gives workers 20\% of the initial video and the related action sequence and the high-level intent of the full video. Workers should do some judgement on six action sequences based on the above information. They only need to choose "True" or "False" of each action sequence.
% The crowdsourcing workers are provided with 20\% of the initial video and the related action sequence. They are required to select the most reasonable choice in the given 6 choices of future action sequences along with the high-level intent, which can correctly reflect the prediction based on the given video. The only difference is that the high-level intent of a video is given. We hope workers will select the most proper future action sequence according to 20\% of the initial video and the related action sequence.
\paragraph{Quality Check via Crowd-Sourcing.} We hired three turkers per video on Amazon Mechanical Turk to check the quality of all answers. For each video, a turker is presented with the first 20\% of the video, two future-directed intents, which are paired with six answer candidates each (an original action sequence and five generated ones), because there were two students working on each video. Turkers are instructed to choose the most reasonable pair of intent and action sequence from all possible combinations. 

We take a few measures to ensure the quality of the answers to multi-choice questions. First, we invited only the turkers who show a certain degree of commitment to this task. We started with publishing a small set of example tasks on AMT. The turkers who are interested are instructed to send us emails. We replied to their emails by providing more detailed instructions and clarifications regarding their mistakes on the trial tasks. The turkers, who demonstrated a good understanding of our task and made no or few mistakes, were invited to work on the full task set. Second, JavaScript based validation tools are applied to make sure that i) turkers start selecting answers after the video plays to the end; ii) only one answer is chosen as the most reasonable one for each question. Third, we published tasks in multiple batches for a continuous quality control. Only the HITs, which are completed by well following our instructions, got paid. The annotation quality control details can be found in \ref{appendix:crowdsourcing_control}.

After checking the answers of all questions in the test set, we applied a set of heuristic rules to determine the final answer to each question. More details can be found in Appendix \ref{appendix:crowdsourcing_rule}. We calculate inter-annotator agreement by asking a group of students, who are not authors, to work on a sample of multi-choice questions of the test set. The corresponding Kappa coefficient \cite{kraemer2014kappa} is 0.91, which demonstrates the high quality of the test set.

Table \ref{table:Statistics of tasks} shows the basic statistics of the test set. The averaged number of observed actions in $\vs$ is similar to the averaged number of future actions. Although all actions in the test appear in the training set, the most plausible action sequences of almost 400 videos are unseen in the training set. This poses a challenge not only for the generalization of multimodal matching but also for compositional generalization. %While splitting the videos into 20\% observed and 80\% unseen, we take into account the average number of observed actions that start before the observed end time of the video and the average number of predicted actions that start after the observed end time.
\begin{table}[h]
%\vspace{-1ex}
\begin{adjustbox}{width=\columnwidth}
\begin{tabular}{l|cc}
\hline
%\multirow{2}{*}{Name} & \multicolumn{}{}{\multirow{}{}{}}  \\
% & \multicolumn{}{c}{} &  \\ \hline
Statistics & Value \\ \hline
\# of videos & 510 \\
    avg. \# of observed actions & 2.79 \\
    avg. \# of future actions & 2.40 \\
    avg. \# of actions  & 5.19 \\
%    \# of choices & 6 \\
%    \# of answers & 1\\
    \# of full action seq occurring in the training set &121 \\
%    \# of intent & 1\\
\hline
\end{tabular}
\end{adjustbox}
\caption{Basic statistics of the test set.}
\label{table:Statistics of tasks}
\vspace{-2ex}
\end{table}

% \begin{table}[]
%     % \centering
%     \scalebox{0.5}{\begin{tabular}{|c|c|c|}
%     \hline
%      & Human Action Forecasting & Human Action Planning \\ \hline
%     Question    & observed 20\% video clip & observed 20\% video clip and textual intent sequence \\ \hline
%     Answer     & textual future action sequence(1 or 2) & textual future action sequence(only 1) \\ \hline
%     Choices & 6 given & 6 given \\ \hline 
%     \end{tabular}}
%     \caption{Comparison of the two tasks.}
%     \label{tab:comp}
% \end{table}
% \subsection{Activity Forecasting}
% \paragraph{\textbf{Overview}} We present this sub-task as Human Activity Forecasting, challenging the current vision \& language systems to understand the temporal actions in human daily activities. We let the system observe the part within 20\% of the initial video clip length and then choose the probable future action sequences from 6 candidates which can represent the future activity that may occur after the given video clips.

% % Different from the previous task, \textbf{action sequence forecasting} \cite{ng2020forecasting}, we evaluate the system performance by providing challenging action sequence choices instead of comparing them with the ground truth action sequence. We argue that those forecasted future action sequence outputs are unnecessarily wrong based on the given video frames. 

% % Now we formulate this task by letting the system observe the part within 20\% of the initial video clip length and then choose the probable future action sequences from 6 candidates which can represent the future activity that may occur after the given video clips. In the process of crowdsourcing, we found there existed more than one action sequence that may occur based on the first 20\% of the video. So we 
% % divided our test videos into single and multiple true future action sequences. Finally, there are 435 videos for the single-answer forecasting task and 75 videos for the multiple-answers forecasting task. 
% \begin{figure}[]
%     \centering
%     \includegraphics[width=.7\linewidth]{diagrams/negative_answer.png}
%     \caption{The cut-off effect was investigated in 510 videos of the test dataset. As shown above, most of the action sequence in 80\% have a length no more than 3, illustrating the importance of adding another method, \textif{Random Addition} to the fake answer generation.}
%     \label{fig:cut_off}
% \end{figure}

% \paragraph{\textbf{Crowdsourcing.}} The crowdsourcing workers are provided with 20\% of the initial video and the related action sequence. They are required to judge if each one in the given 6 choices of future action sequences can correctly reflect the prediction based on the given video.
% % A screenshot of the planning task is given in figure 7.

% \paragraph{\textbf{Negative answers}} Following by \cite{zellers2019recognition}, we adopt the \textbf{Adversarial Matching}, a QA assignment algorithm, to our negative action replacement for the generation of the answer. As our task is to select the reasonable action sequences which can well present the future actions in the given videos, we randomly chose one of the actions in the ground truth future action sequence and replaced it with action from Charades action classes which was relevant enough but not overly similar to the ground truth. Statically, we concluded that the quality of crowd-sourced result achieve the best when $\lambda = 0.7$ in 
% \begin{equation}
% W_i_j=log(P_{rel}(r_i,c_j))+\lambdalog(1-P_{sim}(c_i,c_j))
% \end{equation}
% where $w$ is a
% weight matrix of maximum-weight bipartite matching, $P$ is $P(BERT)$ \cite{devlin2018bert} for $P_{rel}$ and $P_{sim}$ for reference action $r$ and candidate action $c$.


% In the ideal setting of the task, the first $20\%$ video clip should be cut off. After the investigation on the "cut-off" effect in Figure \ref{fig:cut_off}, we found 163 videos out of 510 would only keep 1 action in the remaining $80\%$ video clip while 160 videos have 2 actions after the cut. Hence, we argue that Adversarial Matching is not effective enough when there are no pre-action and post-action around the action to be replaced. \textbf{Random Addition} is suggested in this situation, where we randomly insert one of the actions in the original 157 Charades action classes to the action sequences. We shuffle between the method between \textbf{Adversarial Matching} and \textbf{Random Addition} during the five negative answer construction, which increases the diversity of the negative answers. However, due to the uncertainty of the action recognition approach in Charades, we experimentally find that some of these negative action flows are more suitable for the given videos. Hence, we design our crowd-sourcing task to select two reasonable action flows in the set of ground truth and five "negative" answers. However, due to the high quality of the generated fake answers and various possibilities of prediction. The human experts manually select multiple ground-truth answers for each video in order to control the task quality.
% \subsection{Activity Planning}
% 0.5 page


%The question is the same as in Task 2, but there are no choices provided, and the aim of this task is to match and search with the KG and find the correct action phrase for the hidden video clip.



